DEFORM: A Practical, Universal Deep Beamforming System

We introduce, design, and evaluate a set of universal receiver beamforming techniques. Our approach and system DEFORM, a Deep Learning (DL) based RX beamforming achieves significant gain for multi antenna RF receivers while being agnostic to the transmitted signal features (e.g., modulation or bandwidth). It is well known that combining coherent RF signals from multiple antennas results in a beamforming gain proportional to the number of receiving elements. However in practice, this approach heavily relies on explicit channel estimation techniques, which are link specific and require significant communication overhead to be transmitted to the receiver. DEFORM addresses this challenge by leveraging Convolutional Neural Network to estimate the channel characteristics in particular the relative phase to antenna elements. It is specifically designed to address the unique features of wireless signals complex samples, such as the ambiguous $2\pi$ phase discontinuity and the high sensitivity of the link Bit Error Rate. The channel prediction is subsequently used in the Maximum Ratio Combining algorithm to achieve an optimal combination of the received signals. While being trained on a fixed, basic RF settings, we show that DEFORM DL model is universal, achieving up to 3 dB of SNR gain for a two antenna receiver in extensive experiments demonstrating various settings of modulations, bandwidths, and channels. The universality of DEFORM is demonstrated through joint beamforming relaying of LoRa (Chirp Spread Spectrum modulation) and ZigBee signals, achieving significant improvements to Packet Loss/Delivery Rates relatively to conventional Amplify and Forward (LoRa PLR reduced by 23 times and ZigBee PDR increased by 8 times).

==> discussion.tex <==
\section{Discussion}
\ignore{While the Deep Learning model developed in \system{} is fast, it is still challenging to satisfy the real-time requirements for massive wideband RF data, as one RF sample captured over 1 MHz bandwidth is only \SI{1}{\unit{\micro\second}}  long. As shown in~\Cref{tab:benchmark}, the model prediction is the bottleneck that affects the overall runtime of the pipeline. However, in cases when channels are slowly varying (i.e., stable within a window of hundreds of milliseconds), it is acceptable to reuse the same prediction for a number of chunks of RF samples. For example, using a prediction for 5 chunks of 128 RF samples collected over \SI{1}{\unit{\mega\hertz}} bandwidth (which has a total duration of \SI{0.64}{\unit{\milli\second}}) allows a realtime operation of the system.}

It is clearly seen that the Deep Learning-based approach of \system{} can be extended to larger multi-antenna systems to achieve even higher than 3 dB gain. For a RF receiver system of $N$ receiving antenna elements, the deep learning architecture can be modified to have $2\times(N-1)$ outputs in which two estimations are made for each relative phase offset between the reference antenna and one other antenna. The new requirement of such systems are time synchronization mechanisms for RX radios as typical wireless peripherals have a limited number of antennas (Most of Ettus's USRPs only support 2 simultaneous RX channels \cite{ettus}).

Our current system assumes that there is only one user in the observing spectrum at any given time. The problem becomes more challenging when multiple users are simultaneously transmitting on the same frequency band, which results in significant interference that damages the phase structure in the captured RF samples. In this case, the prediction could be accurate for only one user, or even not working for any users. It would be interesting to investigate the CNN's capability for multi-band spectrum and collision analysis in the future work.

\begin{table}
\centering
\small
  \begin{tabularx}{0.93\linewidth}{|c|c|c|c|c|}
    \hline
    \multirow{2}{2em}{} & \multicolumn{4}{c|}{\textbf{Packet Loss Rate (\%)}}\\
    \cline{2-5}
    Index & Direct & Antenna 1-RL & Antenna 2-RL & \system{}-RL\\
    \hline
    1 & 100 & 22.33 & 11.65 & \textbf{0.97}\\
    2 & 100 & 4.85 & 20.45 & \textbf{2.91}\\
    3 & 100 & 20.39 & 12.91 & \textbf{8.74}\\
    4 & 100 & 16.67 & 7.84 & \textbf{0.98}\\
    \hline
\end{tabularx}
  \caption{Comparison of Packet Loss Rate for LoRa direct and relay (RL) communications.}
  \label{tab:lora_plr}
\end{table}


\begin{table}
\centering
\small
  \begin{tabularx}{0.93\linewidth}{|c|c|c|c|c|}
    \hline
    \multirow{2}{2em}{} & \multicolumn{4}{c|}{\textbf{Packet Delivery Rate (\%)}}\\
    \cline{2-5}
    Index & Direct & Antenna 1-RL & Antenna 2-RL & \system{}-RL\\
    \hline
    1 & 0 & 57.53 & 54.11 & \textbf{77.4}\\
    2 & 0 & 63.01 & 8.22 & \textbf{70.55}\\
    3 & 0 & 21.92 & 15.75 & \textbf{42.47}\\
    4 & 0 & 73.97 & 21.23 & \textbf{76.03}\\
    5 & 0 & 26.03 & 0 & \textbf{39.73}\\ 
    6 & 0 & 47.94 & 28.08 & \textbf{75.34}\\    
    
    \hline
\end{tabularx}
  \caption{Comparison of Packet Delivery Rate for ZigBee direct and relay (RL) communications.}
  \label{tab:lora_plr}
\end{table}

% \begin{table}[t]
% \small
% \centering
%   \begin{tabularx}{0.5\linewidth}{lr}
%     \toprule
%     Module & Runtime\\
%     \midrule
%     Data capturing & 0.047 ms\\
%     Model prediction & 0.566 ms\\
%     Estimation stabilizing & 0.006 ms\\
%     Signal combining & 0.016 ms\\
%     \bottomrule
% \end{tabularx}
%   \caption{Real-time microbenchmark for data of 128 samples.}
%   \label{tab:benchmark}
% \end{table}


